Generating Representative Samples for Few-Shot Classification

Few-shot learning (FSL) aims to learn new categories with a few visual samples per class. Few-shot class representations are often biased due to data scarcity. To mitigate this issue, we propose to generate visual samples based on semantic embeddings using a conditional variational autoencoder (CVAE) model. We train this CVAE model on base classes and use it to generate features for novel classes. More importantly, we guide this VAE to strictly generate representative samples by removing non-representative samples from the base training set when training the CVAE model. We show that this training scheme enhances the representativeness of the generated samples and therefore, improves the few-shot classification results. Experimental results show that our method improves three FSL baseline methods by substantial margins, achieving state-of-the-art few-shot classification performance on miniImageNet and tieredImageNet datasets for both 1-shot and 5-shot settings. Code is available at: https://github.com/cvlab-stonybrook/fsl-rsvae.

==> anlysis_1shot.tex <==

\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=0.4\linewidth]{latex/figs/teaser.png}
\end{center}
\caption{
% 
\textbf{One-shot classification accuracy with different support image-- }
FSL methods heavily depend on how representative the support samples are. The figure shows the one-shot accuracy of the Meta-Baseline method and our method when using 5 different support images whose $L_{2}$ distances to the mean feature of the class "X" ranged from 0.5 to 0.7. The accuracy fluctuates from 72\% to 32\% for Meta-Baseline when using different support images.
}
\label{fig:one-shot}
\end{figure}


\section{One-shot classification accuracy with different support image}
\label{sec:one-shot}


\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=0.5\linewidth]{latex/figs/one-shot.png}
\end{center}
\caption{
% 
\textbf{One-shot classification accuracy with different support image-- }
FSL methods heavily depend on how representative the support samples are. The figure shows the one-shot accuracy of the Meta-Baseline method and our method when using 5 different support images whose $L_{2}$ distances to the mean feature of the class "X" ranged from 0.5 to 0.7. The accuracy fluctuates from 72\% to 32\% for Meta-Baseline when using different support images.
}
\label{fig:one-shot}
\end{figure}

==> idea_bak.tex <==
We use CVAE to obtain unbiased class prototypes.

To make it unbiased, we only use points closer to the class center to train the CVAE.

In training, we pick samples far from the class center as support samples

1 batch: 4x16x5 samples: 16 samples from 1 class for each class with 5 classes:
- randomly 1 as support, and 15 as query
- proposed: select the furthest one as support

W*X
W - the support feature $F_S$
X - the query $F_Q$

objective functions:

we want to choose the hard features as W because we want to increase inter-class distances 

If we train a classifier, we fix the class center, so we try to make all features to get closer to a single vector --> easy to be overfit
we tend to optimize the easy samples rather than the hard-samples.


Here, the hard samples play an important role.
Hard samples are non-representative ones. We want to learn features from these samples more effectively.


Basically, reducing maximum intra-class distance is the key, it reduces the chance of picking a non-representative point as support feature during testing.

We see that, the maximum intra-class distances behaves similarly between the base and novel under different training trials.

The key to reduce the max distance is to force the F.E to learn more from these samples.

We basically do this via adaptive sampling, weighting.


After we train F.E., we use the support feature as prototype.

Attribute is non-biased

What the visual feature provide, even with just one single sample, that the VAE cannot provide.

VAE learns certain relationship between visual features and the attributes. As the attribute space shared between base and novel, these relations generalize to novel.

What F.E. generalizes but VAE can't and vice versa




support: 63
VAE: 66
Combined: 72




Visual data can be challenging to collect and costly to annotate. Few-shot learning (FSL) methods alleviate this data dependency issue by learning visual categories from just a few examples. 


 category name, textual descriptions, or attributes.
 
Data annotations can be in the forms of pixel-level, image-level, or simply class-descriptions. \Hieu{Text descriptions or frequency-based attribute vectors?}

-low-evel supervision vs high-level supervision: 
 
 +concrete vs abstract
 
 +easy to formulate the learning objective vs hard 
 
 +in FSL, high-level supervision plays an important role, but have not been used effectively
 
 
 %Moreover, these methods need to construct the biased prototypes for training, oftenly via meta-learning.   

%Learning such an adaptive correction model is challenging since. % enhance the representativeness of the prototypes obtained via few-shot samples.% correction models that correct the bias in the given few-shot samples using the semantic attributes. 
 %many FSL methods aim to obtain a representative representation for each few-shot class. 
%Estimating the true distribution of data requires a large amount of samples. A typical image training set \cite{Deng2009ImageNetAL,matchingnet,Ren2018MetaLearningFS_tieredImagenet} includes hundreds of samples to fully reflect the key characteristics of the category and various intra-class variations. 

%In FSL where we only have access to a few samples, the classifier tends to overfit the biased distribution formed by the few available samples.

%Many FSL methods aim to enhance the representativeness or correct the biased representations of the few-shot classes \cite{Yang2021FreeLF,JingyiICCV21}.
% biased distribution of each new class formed by a few available examples. It ... 
%the classifier learns to recognize a new category with just a few samples,. These few-shot samples represent a biased distribution of the true data.
%FSL methods in general aim to enhance the representativeness of the few-shot class representation and correct the biased distribution consisting of the few-shot samples \cite{Yang2021FreeLF}. 

%the representiveness of the available samples play the deciding role to the performance of the classifier (see Sec.). 
%the few selected support set samples might be biased.
%a classifier trained on a small set of non-representative data tend to overfit on them and fail to generalize to the testing cases.



%. For example, Fig.\ref{fig:teaser} plots the one-shot accuracy of the Meta-Baseline \cite{metabaseline} method for class ``X'' \todo{fill} of the mini-ImageNet dataset \todo{cite dataset}. The accuracy fluctuates from 72\% to 32\% where an atypical few-shot sample can dramatically reduce the performance.

%Some examples images are visualized in Fig.\ref{fig:teaser} for class ``X''.




%Many few-shot learning algorithms focus on developing stronger models to obtain a more discriminative embedding space, with well-defined distance metrics \cite{protonet, matchingnet, relationnet} or regularization techniques.
%
%Although remarkable performance improvements have been made by these methods, they overlook an important issue in few-shot learning: the few selected support set samples might be biased and can hardly represent the ground truth distribution of the belonging classes.
%Consequently, the classifier trained on these biased data tend to overfit on them and fail to generalize to the testing cases, which are sampled from the ground truth distribution. 



%However, to approximate an unbiased distribution without any prior knowledge is difficult. Semantic information, which is learned from large unsupervised text corpora and independent from visual representations, can provide strong prior knowledge without sample bias. Consider one bird species ``Sternidae" as an example, some images of Sternidae might have blue sky as the background. When these images are selected as the training examples to train a few-shot classifier, the classifier might easily associate ``blue sky" with Sternidae as a discriminative attribute. Such a classifier will fail when the testing images have birds standing on the beach instead of flying in the sky. On the other hand, those semantic information such as ``black forehead", ``orange leg" are representative for this class and universal across different instances. Utilizing these semantic information can help to alleviate the sample bias issue and find the representative features for each class.
%benefit few-shot classification.

%Exploiting the usage of semantic information in few-shot learning has achieved promising improvements in previous works. Zhang \textit{et al.} \cite{zhang2021prototype} propose a prototype completion network to recover representative prototypes by using primitive knowledge and attribute features as priors. Chen \textit{et al.} propose AM3 \cite{}, which modifies the prototype representation of each class by combining information from visual and semantic modalities. 
%Peng \textit{et al.} adaptively intergrate the visual information and the prior knowledge to infer the final classifier for the novel classes. 
%These approaches mainly focus on how to use semantic information to correct the original prototype estimated from the few selected novel samples. However, such correction largely depends on which few-shot samples are given. Learning such a correction model that works well for any given instance is challenging since the within-class variations for the novel classes is generally large.





      \subsection{Zero-shot learning}
      
      \cite{matchingnet,protonet,relationnet,Ye2020FewShotLV,Yang2021FreeLF,Tian2020RethinkingFI,Zhang2020DeepEMDFI} utilize the similarities between images to regularize the embedding space. % by mapping them into a common embedding space. 
      %
      %The derived embedding space is expected to be discriminative, i.e, feature representations from the same object class are grouped together.
      %
      Matching Networks \cite{matchingnet} use an attention mechanism over a learned embedding of the labeled set of examples to predict classes for the unlabeled points.
      %
      The Prototypical Network \cite{protonet} learns to classify query samples based on their Euclidean distance to prototype representations of each class.
      %
      Sung \textit{et al.} \cite{relationnet} propose to measure the distance metric with a CNN-based relation module.
      %
      
      \subsection{Few-shot learning with semantic attributes} 
      \cite{Tokmakov2019LearningCR} proposes a simple attribute-based regularization approach to learn compositional image representations.
      %
      Peng \textit{et al.} \cite{Peng2019FewShotIR} adaptively intergrate the visual information and the prior knowledge to infer the final classifier for the novel classes. 
      %
      Hu \textit{et al.} \cite{Hu2019WeaklysupervisedCF} proposed a compositional feature aggregation module to explore both spatial and semantic visual attributes for FSL.
      
      \cite{zhang2021prototype} xxx
      
      \cite{Xing2019AdaptiveCF_AM3} xxx
      
      \subsection{Sample selection} \cite{dagan,delta-encoder,wang2018lowshot} generate additional training examples to alleviate the problem of data insufficiency. 
      %
      DAGAN \cite{dagan} uses conditional generative adversarial network (GAN) to transform image features, which can be applied to novel unseen classes of data.
      %
      Wang \textit{et al.} \cite{wang2018lowshot} propose to combine a meta-learner with a hallucinator, which can effectively hallucinate novel instances of new classes. Some methods transfer intra-class variance from the base classes to the novel class. The $\Delta$-encoder \cite{delta-encoder} extracts transferable intra-class deformations from image pairs of the same class and uses them to augment samples of the novel classes.
      Differently, our method learns a common distribution of the intra-class variability without pairing any images.
      %
%      \subsection{Transfer Learning}
%     Transfer learning techniques try to transfer the knowledge from some previous tasks to a new task \cite{transfer_one_class,transfer_survey}.     A key issue for transfer learning is “what to transfer”, e.g., which learnt components can be transferred across tasks.
%     In \cite{feature_transfer}, the distribution of feature variance is transferred from regular classes to under-presented classes to address the issue of imbalanced training data.
%     Sun \textit{et al.} propose MTL \cite{meta-transfer}, which transfers pre-trained weights learned on large-scale datasets and aims to meta-learn how to transfer effectively.
%     Hariharan \textit{et al.} \cite{hallucinate_features} present a way of ``hallucinating'' additional examples for novel classes by
%     transferring modes of variation from the base classes.
%     They search for the extracted feature vectors of base categories to collect all quadruplets of transformation “analogies” to train a feature generator.
%     Our variational transfer learning method leverages the idea of transferring the intra-class variance, which intuitively generalizes across classes.
%     However, unlike \cite{hallucinate_features} which trains a feature generator separately, we model the intra-class variance distribution of base categories in an end-to-end training manner.
%     By sampling from the distribution repeatedly, we get synthesized features for novel set images.
     %
     %Compared with \cite{hallucinate_features}, our method avoids 
     
 %    \textbf{Variational Auto-Encoder.}
     Our method uses a VAE to model intra-class variance. VAEs have been used in FSL \cite{variational_fewshot,aligned_vae,proto_vae}.
     %\textbf{Variational Inference in FSL}
     %Variational inference aims to estimate the true distribution of some latent variables in a probabilistic manner.
     %
     %It has been widely used in generative models \cite{vae,beta_vae}, i.e, variational autoencoders (VAE) to produce diverse outputs.
     %
     %Recently, it has also been explored in discriminative models \cite{variational_fewshot,aligned_vae,proto_vae} on few-shot scenarios as well as metric learning problems\cite{metric_learning}.  
     %
   Zhang \textit{et al.}  \cite{variational_fewshot} estimate a distribution for each class and compute the probability of a
     novel input to perform classification.
     %
     Schonfeld \textit{et al.} \cite{aligned_vae} learn a shared latent space of image features and class embeddings via aligned VAEs.
     Instead of modeling the whole image feature, we only use variational inference to model the intra-class variance for our data augmentation framework. The concept of feature disentanglement using VAEs has been used in various applications such as person re-identification \cite{reid2019chanho,Zou2020JointDA}, metric learning \cite{metric_learning}, or multi-domain image translation \cite{unified2018liu,diverse2018lee}.
     We are the first to propose such a VAE-based feature disentanglement scheme for FSL problems. We show that such a model trained on base classes can be used to effectively augment data for the novel classes and significantly improve the classification results.  
     
     
     
     
%Generating diverse data ith large intra-class variance is a challenging problem itself. Here we are more intersted in the representative data ... that greatly benefit FSL classifiers...


 %More importantly, we propose a novel method to improve the representativeness of the generated samples via selecting only representative samples for training our feature generator. 
 %The represenattiveness of samples play an crucial role in constructing few-shot classifier, especially for the prototype-based.
  
 
 %Here, we refer representative samples as ones that lie close to the class center in the feature embedding space and reflect the key characteristics of the category (see Figure \ref{fig:teaser}).
 
 %We find that using this set of the original training data  less data, generate features that lie closer to the real novel class centers. These generated features greatly benefit the few-shot classifier and further improve the performance of our method.


%More importantly, we propose a novel method to improve the representativeness of the generated samples via sample selection. 


%As each category has a semantic representation and a visual representation of image samples. 
%Specifically, %We propose directly generating visual features from the corresponding semantic embeddings. The underlying assumption here is that the projection mapping from a semantic embedding to a distribution of visual features generalizes across all classes. Once we can estimate the mapping via sufficient data in the base classes, we can use the trained model to generate features for novel classes the semantic codes of these new classes. 
%Specifically, we  use as our feature generator a  variational autoencoder (VAE) model. This VAE is trained to generate visual features conditioned on the corresponding semantic embedding of each class. Thus it learns to associate a distribution of features to a conditioned semantic code. Here we assume that such association generalizes across base and novel classes. After training the model using sufficient data from the base classes, we use the trained VAE to generate features for the novel classes and use these generated features together with the few-shot samples to train the classifier. We show that this simple strategy achieves state-of-the-art results on both miniImageNet and tieredImagenet datasets. %Compared to previous FSL methods using semantic information, our method works independently from few-shot samples. 
%It works extremely well for 1-shot scenarios where our method outperforms state-of-the-art methods by 5$\sim$6\% in terms of classification accuracy.
%In spirit, our approach is similar with some zero-shot learning feature generation methods \cite{Guo2021ANP,Ba2015PredictingDZ,Zhang2017LearningAD}. We are the first to propose it for FSL classification problems.

%The classifier trained with our generated features alone achieves better results than many one-shot classifiers (see Sec.). %While this simple strategy is similar to some in zero-shot learning (ZSL) \todo{cite}, we are first to apply it for FSL classification.

%Essentially, we aim to capture the correlations between visual features and semantic attributes using those samples from the base classes. We find that this correlation


%\todo{cite paper that tried it but got bad results}.

%This feature generation approach is simpler and better since the generated features are only conditioned on the semantic information, which naturally encodes class-representative features and is independent from any few-shot visual instances. 
%model a distribution of representative features for each class. This strategy 
%class-representative.   features and is independent from visual instances. 

%Synthesizing visual features using semantic information to help image classification has been mostly driven by zero-shot learning (ZSL), which aims at recognizing categories whose instances have not been seen during training. 
%In ZSL, a generative adversarial network (GAN) is mostly used in conjunction with a VAE to optimize the divergence between real and generated data.
%In ZSL, the generated features are desired to be more diverse, which is aligned with the distribution of real features. Feature generation for few-shot learning, on the other hand, aims to find the representative points for each class to alleviate the sample bias issue. Therefore, directly applying feature synthesis methods designed for ZSL on few-shot learning might degrade the performance.

%Due to the diversity of the image data, not all the visual features sharing the same class label encode class-representative information. For instance, an image of a person carrying a dog will still be annotated as a dog, although the person might occupy majority part of the image. Those non-representative features are not desirable for finding a reliable class prototype. 

%To this end, we propose a variational autoencoder (VAE) based framework to generate representative features using the corresponding semantic information to alleviate the sample bias issue in few-shot learning. 
%More importantly, we propose a method to  enhance the representativeness of the generated features and further improve the few-shot classification performances. 

 %In essence, we use the proposed VAE model to learn the correlation between a semantic embedding and a distribution of visual features. However, not all the visual samples encode class-representative information that aligns with the semantic embedding. For instance, an image of a person holding a dog would still be annotated as a dog, although the person might occupy majority part of the image, as visualized in Figure \ref{fig:teaser}. These non-representative samples effectively hinder the model's ability to precisely align the semantic embedding to the relevant visual features. To mitigate this issue, we propose to only use a subset of representative features to train the VAE model. 
 
 
%Here in FSL, we 

%However, not all images of a category is class-representative. For instance, an image of a person holding a dog would still be annotated as a dog, although the person might occupy majority part of the image (Figure \ref{fig:teaser}). In conventional learning problems, these non-representative samples diversify the dataset and present various intra-class variations that benefit training a classifier. However, in FSL settings where we aim to construct a representative prototype for each novel class, we are generally more interested in the set of representative samples which lie close to the class center.
 
 
 
 
 %We show that the generated features using the VAE can alleviate the sample bias issue effectively regardless of the selection of the few-shot samples. 
 
 %

==> relatedwork.tex <==

Learning from auxiliary 

VAEs have been widely used in Zero-Shot Learning (ZSL) where we assume that no image of novel classes is available during training.  ZSL methods thus rely on an auxiliary modality containing some information of the unseen classes such as textual descriptions [more papers] or attribute vectors \cite{Devise_13} and focuses on learning the relationship between the visual and the auxiliary domains. For example, Frome \etal propose using a semantic embedding space to 

The concept of aligning the semantic embedding space and the visual embedding space has been used in some ZSL methods \cite{Devise_13}. Tsai \etal propose to learn joint embeddings for semantic and visual features in which they align the feature distributions between the two domains.

However, it is not trivial to simply apply them to a few-shot learning setting.   

\cite{Huang2021AGAM}

xx aims to associate pre-trained visual feature
representations to each attributes via 

Adaptive Cross-Modal Few-shot Learning

Generalized Zero- and Few-Shot Learning via Aligned Variational Autoencoders
